A low-cost four-component relativistic coupled cluster linear response theory based on perturbation sensitive natural spinors

We present an efficient implementation of four-component linear response coupled cluster singles and doubles (4c-LRCCSD) theory that enables accurate and computationally efficient calculation of polarizabilities for systems containing heavy elements. We have observed that the frozen natural spinor (FNS)-based truncation scheme is not suitable for linear response properties, as it leads to larger errors in static and dynamic polarizability values. In this work, we have introduced a "perturbation-sensitive" density to construct the natural spinor basis, termed FNS++. Using FNS++, we achieve excellent accuracy when compared to experimental data and other theoretical results, even after truncating nearly 70% of the total virtual spinors. We also present pilot applications of 4c-LRCCSD with a canonical basis to calculate the polarizability spectra of 3d transition metals. By employing the FNS++-based 4c-LRCCSD, we have been able to compute polarizabilities for systems with over 1200 virtual spinors, maintaining low computational cost and excellent accuracy.

==> aiptemplate.tex <==
%%
%% This is file `ltxdocext.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% ltxdocext.dtx  (with options: `package,kernel')
%% 
%% This is a generated file;
%% altering it directly is inadvisable;
%% instead, modify the original source file.
%% See the URL in the file README.
%% 
%% License
%%    You may distribute this file under the conditions of the
%%    LaTeX Project Public License 1.3 or later
%%    (http://www.latex-project.org/lppl.txt).
%% 
%%    This file is distributed WITHOUT ANY WARRANTY;
%%    without even the implied warranty of MERCHANTABILITY
%%    or FITNESS FOR A PARTICULAR PURPOSE.
%% 
\NeedsTeXFormat{LaTeX2e}[1995/12/01]%
\ProvidesFile{ltxdocext.sty}%
 [2008/08/04 1.1b2 ltxdoc extensions package]% \fileversion
\def\class@name{ltxdocext}%
\expandafter\PackageInfo\expandafter{\class@name}{%
 An extension to the \protect\LaTeXe\space ltxdoc class
 by A. Ogawa (arthur\_ogawa sbcglobal.net)%
}%
\RequirePackage{verbatim}%
\let\o@verbatim\verbatim
\def\verbatim{%
  \ifhmode\unskip\par\fi
  \ifx\@currsize\normalsize
     \small
  \fi
  \o@verbatim
}%
\renewcommand \verbatim@font {%
  \normalfont \ttfamily
  \catcode`\<=\active
  \catcode`\>=\active
}%
\RequirePackage{shortvrb}
\AtBeginDocument{%
 \MakeShortVerb{\|}%
}%
\begingroup
  \catcode`\<=\active
  \catcode`\>=\active
  \gdef<{\@ifnextchar<\@lt\@meta}
  \gdef>{\@ifnextchar>\@gt\@gtr@err}
  \gdef\@meta#1>{\marg{#1}}
  \gdef\@lt<{\char`\<}
  \gdef\@gt>{\char`\>}
\endgroup
\def\@gtr@err{%
   \ClassError{ltxguide}{%
      Isolated \protect>%
   }{%
      In this document class, \protect<...\protect>
      is used to indicate a parameter.\MessageBreak
      I've just found a \protect> on its own.
      Perhaps you meant to type \protect>\protect>?
   }%
}
\def\verbatim@nolig@list{\do\`\do\,\do\'\do\-}
\def\GetFileInfo#1{%
  \def\filename{#1}%
  \def\@tempb##1 ##2 ##3\relax##4\relax{%
    \def\filedate{##1}%
    \def\fileversion{##2}%
    \def\fileinfo{##3}}%
  \edef\@tempa{\csname ver@#1\endcsname}%
  \expandafter\@tempb\@tempa\relax? ? \relax\relax}
\DeclareRobustCommand{\marg}[1]{%
 \meta{#1}%
 \index{#1=\string\meta{#1} placeholder}\index{placeholder>#1=\string\meta{#1}}%
}%
\DeclareRobustCommand\meta[1]{%
 \mbox{\LANGLE\itshape#1\/\RANGLE}%
}%
\def\LANGLE{$\langle$}%
\def\RANGLE{$\rangle$}%
\DeclareRobustCommand{\arg}[1]{%
 {\ttfamily\string{}\meta{#1}{\ttfamily\string}}%
 \index{#1=\string\ttt{#1}, argument}\index{argument>#1=\string\ttt{#1}}%
}%
\let\oarg\undefined
\DeclareRobustCommand{\oarg}[1]{%
 {\ttfamily[%]
  }\meta{#1}{\ttfamily%[
 ]}%
 \index{#1=\string\ttt{#1}, optional argument}%
 \index{argument, optional>#1=\string\ttt{#1}}%
}%
\DeclareRobustCommand\cmd{\begingroup\makeatletter\@cmd}%
\long\def\@cmd#1{%
 \endgroup
 \cs{\expandafter\cmd@to@cs\string#1}%
 \expandafter\cmd@to@index\string#1\@nil
}%
\def\cmd@to@cs#1#2{\char\number`#2\relax}%
\def\cmd@to@index#1#2\@nil{%
 \index{#2=\string\cmd#1#2}%\index{command>#2=\string\cmd#1#2}%
}%
\DeclareRobustCommand\cs[1]{{\ttfamily\char`\\#1}}%
\def\scmd#1{%
 \cs{\expandafter\cmd@to@cs\string#1}%
 \expandafter\scmd@to@index\string#1\@nil
}%
\def\scmd@to@index#1#2\@nil#3{%
 \index{\string$#3=\string\cmd#1#2---#3}%
}%
\DeclareRobustCommand\env{\name@idx{environment}}%
\DeclareRobustCommand\envb[1]{%
 {\ttfamily\string\begin\string{}\env{#1}{\ttfamily\string}}%
}%
\DeclareRobustCommand\enve[1]{{\ttfamily\string\end\string{}\env{#1}{\ttfamily\string}}}%
\DeclareRobustCommand{\file}{\begingroup\@sanitize\@file}%
\long\def\@file#1{\endgroup
 {\ttfamily#1}%
 \index{#1=\string\ttt{#1}}\index{file>#1=\string\ttt{#1}}%
}%
\DeclareRobustCommand\substyle{\name@idx{document substyle}}%
\DeclareRobustCommand\classoption{\name@idx{document class option}}%
\DeclareRobustCommand\classname{\name@idx{document class}}%
\def\name@idx#1#2{%
 {\ttfamily#2}%
 \index{#2\space#1=\string\ttt{#2}\space#1}\index{#1>#2=\string\ttt{#2}}%
}%
\DeclareRobustCommand\url@ltxdocext{\begingroup\catcode`\/\active\catcode`\.\active\catcode`\:\active\@url}%
\AtBeginDocument{%
 \ifx\url\undefined\let\url\url@ltxdocext\fi
}%
\def\@url#1{%
 \url@break{\ttfamily#1}%
 \url@char\edef\@tempa{#1=\string\url{#1}}%
 \expandafter\index\expandafter{\@tempa}%
 \expandafter\index\expandafter{\expandafter u\expandafter r\expandafter l\expandafter >\@tempa}%
 \endgroup
}%
{\catcode`\:\active\aftergroup\def\aftergroup:}{\active@colon}%
\def\colon@break{\colon@char\allowbreak}%
\def\colon@char{:}%
{\catcode`\/\active\aftergroup\def\aftergroup/}{\active@slash}%
\def\slash@break{\slash@char\allowbreak}%
\def\slash@char{/}%
{\catcode`\.\active\aftergroup\def\aftergroup.}{\active@dot}%
\def\dot@break{\dot@char\allowbreak}%
\def\dot@char{.}%
\def\url@break{\let\active@slash\slash@break\let\active@dot\dot@break\let\active@colon\colon@break}%
\def\url@char{\let\active@slash\slash@char\let\active@dot\dot@char\let\active@colon\colon@char}%
\renewenvironment{theindex}
               {\if@twocolumn
                  \@restonecolfalse
                \else
                  \@restonecoltrue
                \fi
                \columnseprule \z@
                \columnsep 35\p@
\def\see##1##2{\textit{See} ##1}%
\def\seealso##1##2{\textit{See also} ##1}%
\long\def\cmd##1{\cs{\expandafter\cmd@to@cs\string##1}}%
\def\@url##1{\url@break\ttt{##1}\endgroup}%
\def\ttt{\begingroup\@sanitize\ttfamily\@ttt}%
\def\@ttt##1{##1\endgroup}%
\mathchardef\save@secnumdepth\c@secnumdepth
\c@secnumdepth\m@ne
                \twocolumn[\section{\indexname}]%
\c@secnumdepth\save@secnumdepth
                \thispagestyle{plain}\parindent\z@
                \parskip\z@ \@plus .3\p@\relax
                \let\item\@idxitem}
               {\if@restonecol\onecolumn\else\clearpage\fi}
\renewenvironment{quote}
               {\list{}{%
                \leftmargin1em\relax
                \rightmargin\leftmargin
                }%
                \item\relax}
               {\endlist}
\newif\if@mainmatter
\newif\if@openright
\@openrighttrue
\DeclareRobustCommand\frontmatter{%
  \cleartorecto
  \@mainmatterfalse
  \pagenumbering{roman}%
}%
\DeclareRobustCommand\mainmatter{%
  \cleartorecto
  \@mainmattertrue
  \pagenumbering{arabic}%
}%
\DeclareRobustCommand\backmatter{%
  \if@openright
    \cleartorecto
  \else
    \clearpage
  \fi
  \@mainmatterfalse
}%
\ifx\undefined\cleartorecto
 \def\cleartorecto{\cleardoublepage}%
\fi
\def\@to{to}%
\newenvironment{unnumtable}{%
 \par
 \addpenalty\predisplaypenalty
 \addvspace\abovedisplayskip
 \hbox\@to\hsize\bgroup\hfil\ignorespaces
  \let\@Hline\@empty
}{%
 \unskip\hfil\egroup
 \penalty\postdisplaypenalty
 \vskip\belowdisplayskip
 \aftergroup\ignorespaces
 \@endpetrue
}%
\providecommand\toprule{\hline\hline}%
\providecommand\colrule{\\\hline}%
\providecommand\botrule{\\\hline\hline}%
\DeclareRobustCommand\subsubsubsection{%
 \@startsection{subsubsection}{4}%
  {\z@}{-15\p@\@plus-5\p@\@minus-2\p@}%
  {5\p@}{\normalfont\normalsize\itshape}%
}%
\DoNotIndex{\',\.,\@M,\@@input,\@Alph,\@alph,\@addtoreset,\@arabic}
\DoNotIndex{\@badmath,\@centercr,\@cite}
\DoNotIndex{\@dotsep,\@empty,\@float,\@gobble,\@gobbletwo,\@ignoretrue}
\DoNotIndex{\@input,\@ixpt,\@m,\@minus,\@mkboth}
\DoNotIndex{\@ne,\@nil,\@nomath,\@plus,\roman,\@set@topoint}
\DoNotIndex{\@tempboxa,\@tempcnta,\@tempdima,\@tempdimb}
\DoNotIndex{\@tempswafalse,\@tempswatrue,\@viipt,\@viiipt,\@vipt}
\DoNotIndex{\@vpt,\@warning,\@xiipt,\@xipt,\@xivpt,\@xpt,\@xviipt}
\DoNotIndex{\@xxpt,\@xxvpt,\\,\ ,\addpenalty,\addtolength,\addvspace}
\DoNotIndex{\advance,\ast,\begin,\begingroup,\bfseries,\bgroup,\box}
\DoNotIndex{\bullet}
\DoNotIndex{\cdot,\cite,\CodelineIndex,\cr,\day,\DeclareOption}
\DoNotIndex{\def,\DisableCrossrefs,\divide,\DocInput,\documentclass}
\DoNotIndex{\DoNotIndex,\egroup,\ifdim,\else,\fi,\em,\endtrivlist}
\DoNotIndex{\EnableCrossrefs,\end,\end@dblfloat,\end@float,\endgroup}
\DoNotIndex{\endlist,\everycr,\everypar,\ExecuteOptions,\expandafter}
\DoNotIndex{\fbox}
\DoNotIndex{\filedate,\filename,\fileversion,\fontsize,\framebox,\gdef}
\DoNotIndex{\global,\halign,\hangindent,\hbox,\hfil,\hfill,\hrule}
\DoNotIndex{\hsize,\hskip,\hspace,\hss,\if@tempswa,\ifcase,\or,\fi,\fi}
\DoNotIndex{\ifhmode,\ifvmode,\ifnum,\iftrue,\ifx,\fi,\fi,\fi,\fi,\fi}
\DoNotIndex{\input}
\DoNotIndex{\jobname,\kern,\leavevmode,\let,\leftmark}
\DoNotIndex{\list,\llap,\long,\m@ne,\m@th,\mark,\markboth,\markright}
\DoNotIndex{\month,\newcommand,\newcounter,\newenvironment}
\DoNotIndex{\NeedsTeXFormat,\newdimen}
\DoNotIndex{\newlength,\newpage,\nobreak,\noindent,\null,\number}
\DoNotIndex{\numberline,\OldMakeindex,\OnlyDescription,\p@}
\DoNotIndex{\pagestyle,\par,\paragraph,\paragraphmark,\parfillskip}
\DoNotIndex{\penalty,\PrintChanges,\PrintIndex,\ProcessOptions}
\DoNotIndex{\protect,\ProvidesClass,\raggedbottom,\raggedright}
\DoNotIndex{\refstepcounter,\relax,\renewcommand}
\DoNotIndex{\rightmargin,\rightmark,\rightskip,\rlap,\rmfamily}
\DoNotIndex{\secdef,\selectfont,\setbox,\setcounter,\setlength}
\DoNotIndex{\settowidth,\sfcode,\skip,\sloppy,\slshape,\space}
\DoNotIndex{\symbol,\the,\trivlist,\typeout,\tw@,\undefined,\uppercase}
\DoNotIndex{\usecounter,\usefont,\usepackage,\vfil,\vfill,\viiipt}
\DoNotIndex{\viipt,\vipt,\vskip,\vspace}
\DoNotIndex{\wd,\xiipt,\year,\z@}
\DoNotIndex{\next}
\AtEndDocument{\PrintIndex\PrintChanges}%
\makeatletter
\def\endfilecontents{%
 \immediate\write\reserved@c{%
  \string\iffalse\space ltxdoc klootch^^J%
  \ifx\undefined\fileversion\else
  \ifx\undefined\filedate\else
  This file has version number \fileversion, last revised \filedate.%
  \fi\fi
  \string\fi
 }%
 \immediate\closeout\reserved@c
 \def\T##1##2##3{%
  \ifx##1\@undefined\else
    \@latex@warning@no@line{##2 has been converted to Blank ##3e}%
  \fi
 }%
 \T\L{Form Feed}{Lin}%
 \T\I{Tab}{Spac}%
 \immediate\write\@unused{}%
}%
\expandafter\let\csname endfilecontents*\endcsname\endfilecontents
\makeatother
\setlength\arraycolsep{0pt}%
\endinput
%%
%% End of file `ltxdocext.sty'.
